Computational Spectral Imaging with Unified Encoding Model: A Comparative Study and Beyond

Computational spectral imaging is drawing increasing attention owing to the snapshot advantage, and amplitude, phase, and wavelength encoding systems are three types of representative implementations. Fairly comparing and understanding the performance of these systems is essential, but challenging due to the heterogeneity in encoding design. To overcome this limitation, we propose the unified encoding model (UEM) that covers all physical systems using the three encoding types. Specifically, the UEM comprises physical amplitude, physical phase, and physical wavelength encoding models that can be combined with a digital decoding model in a joint encoder-decoder optimization framework to compare the three systems under a unified experimental setup fairly. Furthermore, we extend the UEMs to ideal versions, namely, ideal amplitude, ideal phase, and ideal wavelength encoding models, which are free from physical constraints, to explore the full potential of the three types of computational spectral imaging systems. Finally, we conduct a holistic comparison of the three types of computational spectral imaging systems and provide valuable insights for designing and exploiting these systems in the future.

==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}
Spectral imaging is a valuable technique that captures both spatial and spectral information of a scene, enabling material discrimination and object classification by analyzing their spectral features. Consequently, spectral imaging has found applications in various fields, such as biology~\cite{li2013review}, medicine~\cite{zeng2022research}, food industry~\cite{qin2013hyperspectral}, art~\cite{balas2003novel}, and agriculture~\cite{mancini2019challenges}. Nonetheless, conventional spectral imaging systems are bulky and require time-consuming scanning to acquire spatial and spectral information, which limits their application in dynamic scenes.
Thus, computational spectral imaging is the most promising solution that can efficiently capture spectral information of dynamic scenes without scanning.

Currently, there are three types of physically implementable computational spectral imaging systems according to their encoding methods: amplitude encoding systems based on compressive sensing~\cite{gehm2007single, august2013compressive, llull2013coded}, phase encoding systems that rely on diffractive optics~\cite{golub2016compressed, 2019Compact, hauser2020dd}, and wavelength encoding systems that employ filters~\cite{nguyen2014training, robles2015single}. These systems capture spectral scenes into a single snapshot measurement using well-designed optical encoders and then reconstruct them using corresponding digital decoders.

% Current works 加几个参考文献
So far, the three types of computational spectral imaging systems have only been developed and studied in their respective fields, highlighting the need to unify them under a common framework for comparative analysis. 
However, the heterogeneity of the three systems makes it impossible to apply the hand-crafted optical design from one type of computational spectral imaging system to another, making the fair comparative analysis challenging. 
% Specifically, in the comparison of current works\cite{huang2022spectral}, the encoding systems proposed by these works are carefully hand-crafted for their own settings, while the compared encoding systems are borrowed from another setting. As the encoding systems are hand-crafted or optimized separately in different settings, the comparison is obviously biased.
Therefore, there is an urgent need for comprehensive and unbiased comparative studies under a unified setting to determine which of the three computational spectral imaging systems is superior.


To comprehensively compare the performance of the three types of spectral imaging systems under a unified and fair setting, we propose the unified encoding model (UEM) can model all the spectral imaging systems.
% 先往宏观说，UEM能够建模所有的光谱成像系统，可以用一个model对三个系统做建模
To represent a specific spectral imaging system, it can be cast to the physical amplitude encoding model (AEM-P), the physical phase encoding model (PEM-P), or the physical wavelength encoding model (WEM-P). 
And we employ the recently proposed joint encoder-decoder optimization approach for computational imaging system~\cite{sitzmann2018end} to optimize the three casted UEMs along with the corresponding decoding models towards the same spectral imaging objective, for comparing the three types of computational spectral systems under the same setting. 
Our proposed UEM provides a macroscopic perspective that encompasses all computational spectral imaging systems within a unified framework. This allows us to gain a comprehensive understanding of these systems from a broader perspective.


% 少体现分，讲太多了，要体现宏观的统一
Furthermore, to fully explore the potential performance of the three types of computational spectral imaging systems in our comparative study, we propose ideal models with greater degrees of freedom that eliminate the constraints of physical models.
These ideal models, including the ideal amplitude encoding model (AEM-I), ideal phase encoding model (PEM-I), and ideal wavelength encoding model (WEM-I), offer an opportunity to push the performance limits of each type of spectral imaging system.
% 不说消除了什么，只说enable了什么
Specifically, the AEM-I model enables the free modulation of amplitude to any possible value (i.e., 32-bit floating point number) in both spatial and spectral dimensions, the PEM-I model enables any form of the point spread function (PSF) to be achieved, and the WEM-I model allows any shape of the spectral response curve to be accepted.
The encoding properties obtained through this high-degree-of-freedom optimization process provide valuable guidance for subsequent encoding design.

%image segmentation
Additionally, to explore the performance of imaging results on high-level tasks, we also conduct spectral image segmentation experiments and observe that there is no positive correlation between segmentation performance and imaging quality.
%character
Through the characterization of each system in the experiment, we gain a more comprehensive understanding of the three computational spectral imaging systems and provide guidance for the development of computational spectral imaging systems.


To summarize, we make several significant contributions:
\begin{itemize}

    \item We propose the UEM for the three types of physically implementable computational spectral imaging systems for comparing them fairly under the unified settings of joint encoder-decoder optimization.
    
    \item We extend the UEMs to the ideal version with greater degrees of freedom by removing the physical constraints of the three models, to fully explore the potential performance of the three types of computational spectral imaging systems.
    
    \item We provide comprehensive comparisons of the performance and potential for the three types of computational spectral imaging systems based on the physical and ideal UEMs, investigate how the low-level imaging performance influences the downstream high-level segmentation task.
    %, and analyze the characteristics of the three types of systems
  
\end{itemize}

==> sec/2_relatedwork.tex <==
\section{Related Work}

%\subsection{Amplitude Encoding System}
\noindent {\bf{Amplitude Encoding System.}} 
The amplitude encoding system is based on the theory of compressive sensing~\cite{donoho2006compressed,wakin2006architecture,candes2008introduction}, which combines optics, mathematics, and optimization theory. This system employs an encoding mask to block or filter the input light and then passes through the dispersion element to acquire an image with compressed information~\cite{duarte2008single,duarte2013spectral,arce2013compressive,martin2014hyca,cao2016computational,oiknine2018compressive}. The image generation is expressed as a point multiplication process between a mask that is consistent with the image size and a monochromatic object image for each wavelength. Finally, a specific reconstruction algorithm decodes and obtains the underlying spectral image.
% While conventional methods based on CASSI tend to use randomly coded apertures, in the amplitude encoding system, the coded apertures are considered encoders with embedded spectral features optimized together with a decoder composed of reconstruction algorithms. 

Wang et al. proposed HyperReconNet~\cite{wang2018hyperreconnet} jointly learns the coded mask and the corresponding CNN for reconstruction. The BinaryConnect~\cite{courbariaux2015binaryconnect} adds the encoded mask to the network as a layer, using a floating-point mapping to the binary-encoded mask entity.
E. Salazar et al.~\cite{salazar2020coded} proposed an optimal coded mask algorithm for the Spatial Spectral Compressive Spectral Imager (SSCSI) based on a discrete measurement model of his own design. 
D2UF~\cite{jacome2022d} encoded the mask and multispectral color filter array (MCFA) of the CASSI system and performed spectral reconstruction using an unrolling-based network.

%
% CASSI can be divided into single dispersive CASSI (SD-CASSI) and dual dispersive CASSI (DD-CASSI) depending on the number of dispersion elements in the CASSI system.
% We choose the SD-CASSI, the most representative of current amplitude encoding systems, as the reference for the AEM-P.

%\subsection{Phase Encoding System}
\noindent {\bf{Phase Encoding System.}} 
The phase encoding system has the advantage of its lightweight and not blocking any incoming light and therefore increasing the light efficiency of the system. In phase encoding systems, diffractive optical elements (DOE)~\cite{taghizadeh1997design} or metasurfaces~\cite{neshev2023enabling} are employed and designed to control the phase modulation in terms of the PSF to act as encoders that collect desired spectral information.

Several research efforts have been made to improve the phase encoding system. Peng et al.~\cite{peng2016diffractive} proposed a shape-invariant PSF design approach for high-quality color imaging, while Jeon et al.~\cite{jeon2019compact} designed a spectrally varying PSF that rotates regularly with wavelength and encodes spectral information. Xiong et al.~\cite{dun2020learned} decomposed the PSF formula into Bessel functions, simplified these functions according to rotational symmetry, and reconstructed the network using a W-Net composed of Res-U-Net units. Arguello et al.~\cite{arguello2021shift} introduced a color-coded aperture (CCA) and designed the spatially variable PSF.

To address the quantization issue of DOE height maps, Li et al.~\cite{li2022quantization} integrated the quantization operation into the DOE optimization process, using an adaptive mechanism to optimize the physical height of each volume layer. Additionally, Tseng et al.~\cite{tseng2021neural} and Makarenko et al.~\cite{makarenko2022real} used metasurface instead of DOE as the encoding element, which also achieved good results.
% The development of advanced PSF design and optimization methods, along with the use of novel encoding elements, has led to significant improvements in the spectral imaging capabilities of the phase encoding system.

% We choose the rotationally symmetrical encoding DOE as a reference for the PEM-P, which is a remarkable breakthrough in phase encoding systems because it both reduces the computational complexity of designing and the difficulties of fabrication.

% \subsection{Wavelength Encoding System}

\noindent {\bf{Wavelength Encoding System.}} 
% Both systems above add specific optical elements in front of the sensor to encode the scene light in a specific way, while 
The wavelength encoding system uses RGB narrowband filters or other band filters directly to encode the scene in the wavelength dimension and then perform spectral reconstruction of the captured image. Since wavelength encoding systems perform no modulation on spatial dimensions, they usually report better spatial quality in the reconstruction result than other encoding systems.

The most common wavelength encoding system directly regards the imaging pipeline of an arbitrary or well-selected RGB camera as the encoding process, i.e., they directly build reconstruction algorithms based on RGB images. 
In 2017, Xiong et al.~\cite{xiong2017hscnn} proposed HSCNN, which applied CNN to upsampled RGB and amplitude-encoded measurements for spectral reconstruction.
In the same year, Galliani et al~\cite{galliani2017learned} proposed a learned spectral super-resolution using CNN for end-to-end RGB to spectral image reconstruction.
The current very popular attention mechanism~\cite{vaswani2017attention} has also been applied in the field of spectral imaging. Cai et al~\cite{cai2022mst++} proposed Transformer-based MST++, which uses cells based on HSI spatial sparsity and spectral self-similarity properties as the base module.

Admittedly, existing RGB narrowband filters are designed to satisfy human vision and they are intuitively sub-optimal for spectral imaging. Therefore, some researchers chose filters to achieve a suitable spectral response for spectral imaging~\cite{fu2020joint}, and some optimized the response to obtain better spectral imaging performance.
Nie, S., et al.~\cite{nie2018deeply} encoded the RGB filter and combined this function with the reconstruction network for end-to-end optimization on the spectral reconstruction task. 

%
% We choose the method of selection of existing response curves of filters in the wavelength encoding system as the reference for the WEM-P.

% \subsection{Joint Encoder-decoder Optimization}
\noindent {\bf{Joint Encoder-decoder Optimization.}}
With the advancements in computational photography, joint encoder-decoder optimization methods have become the mainstream technique to enhance imaging performance.
Instead of designing the encoder and the decoder separately like traditional approaches, the joint encoder-decoder optimization algorithm optimizes both the encoder and decoder simultaneously for a given task.
The superior performance of the joint encoder-decoder optimization method has been demonstrated in various computational imaging tasks such as HDR imaging~\cite{metzler2020deep, sun2020learning} and depth estimation~\cite{ikoma2021depth, baek2021single, liu2022investigating}. 
Also, the joint encoder-decoder optimization has been applied to spectral imaging tasks using amplitude encoding systems~\cite{kobayashi2022compressive,shi2023compact} and phase encoding systems~\cite{dun2020learned, li2022quantization, sun2022hyperspectral}, and there is still a lack of clear understanding regarding the optimal performance of computational spectral imaging systems. 

%
% Due to the superiority of the joint encoder-decoder optimization, we use the joint encoder-decoder optimization algorithm to optimize a casted UEM and corresponding  decoding model for a computational spectral imaging system.

==> sec/3_uem.tex <==
\section{Unified Encoding Model}
We begin with an overview of the UEM, followed by a detailed description of the physical and ideal version of it.


\begin{table}[!t]
  \centering
  \caption{Physical systems corresponding to each physical UEM.}
  \label{table_model}
  \resizebox{\linewidth}{!}
  {\begin{tabular}{cc}
  \hline
    \textbf{Encoding Model} & \textbf{Physical Systems} \\ \hline
    \textbf{AEM-P} & SD-CASSI~\cite{wagadarikar2008single}, 3D-CASSI~\cite{lin2014dual, correa2014compressive, arguello2014colored} \\ 
    \textbf{PEM-P} & Rotationally Symmetric DOE~\cite{dun2020learned}, Free DOE~\cite{baek2021single} \\ 
    \textbf{WEM-P} & Fixed Filter~\cite{cai2022mst++}, Learned Filter~\cite{nie2018deeply} \\ \hline
  \end{tabular}}
\end{table}

\begin{figure}[!t]
\centering
\subfloat[Mask in AEM]{\includegraphics[width=1in]{Figure/MASK_paint.pdf}}
\label{MASK_paint}\hspace{2mm}
\subfloat[DOE in PEM]{\includegraphics[width=1in]{Figure/DOE_paint.pdf}}
\label{DOE_paint} \hspace{2mm}
\subfloat[Filter in WEM]{\includegraphics[width=1in]{Figure/Sensor_paint.pdf}}
\label{Sensor_paint}

\caption{Optical encoding elements in the three casted UEMs.}
\label{fig_optical_element}
\end{figure}



\subsection{Overview}
% Overview
We propose the UEM that covers all three types of optical modulations for spectral imaging, thus we can cast the UEM into AEM, PEM, and WEM to represent amplitude, phase, and wavelength encoding systems respectively.
The corresponding optical encoding elements are shown in Figure~\ref{fig_optical_element}.
Specifically, for amplitude modulation, the scene light is element-wise multiplied with the matrix $A(x,y,\lambda)$ of the encoding mask; 
For phase modulation, the light is convolved with the PSF $P(x,y,\lambda)$ of the DOE; 
For wavelength modulation, the light is multiplied by the spectral response $W(\lambda)$ of the filter, integrated along the wavelength dimension $\lambda$, and converted into a measurement $I_{rgb}$ on the RGB sensor. 
% We give the formula for UEM as follows:
We give the overall formula for the UEM as follows, with some terms becoming unit terms under specific settings:
\begin{equation}
	I_{rgb} = \int W(\lambda) \cdot P(x,y,\lambda) \ast (A(x,y,\lambda)\cdot I(x,y,\lambda) ) d\lambda,
 \label{eq:uem}
\end{equation}	
where $I(x,y,\lambda)$ denotes the natural spectral scene, and $I_{rgb}$ is the RGB encoded image captured by the sensor.

In the following, we introduce two versions of UEMs, the physical version, and the ideal version.
The physical UEM is modeled with physical constraints in the encoding process, which corresponds to a certain series of physically implementable encoding systems for spectral imaging.
Based on the physical UEM, we are able to put the three types of physically implementable spectral imaging systems into one unified setting for comparative study.

Beyond, the ideal UEMs are extended from the physical UEMs by eliminating the physical constraints of the encoding process, which means the ideal UEMs have higher degrees of encoding freedom. 
We employ the ideal UEMs to investigate the maximum potential of each type of spectral imaging system. 
For convenience, we use the suffix `-P' to denote the physical UEMs and the suffix `-I' to indicate ideal UEMs.


% \begin{figure}[!t]
%  \centering
%  \includegraphics[width=\linewidth]{Figure/sdcassi_paint.png}
%  \caption{Optical encoding propagation of SD-CASSI.}
%  \label{sdcassi_paint}
% \end{figure}


\subsection{Physical Model}
We first introduce the physical UEMs and cast them to AEM-P, PEM-P, and WEM-P for physically implementable amplitude, phase, and wavelength encoding systems respectively.
The representative physical systems that correspond to each physical UEM are presented in Table~\ref{table_model}.


\noindent {\bf{Physical Amplitude Encoding Model.}} 
The AEM-P only employs the amplitude modulation part of the UEM, with physical constraints on the modulation that should be implementable using a mask.

SD-CASSI~\cite{wagadarikar2008single} is a widely used physical amplitude encoding system, its optical encoding process is demonstrated in Figure~\ref{fig_uempaint}(a). 
The system uses a 0-1 encoding mask to modulate the spatial amplitude of the incident light, followed by a dispersion element that introduces distinct offsets for varying wavelengths of light, ultimately compressing the spectral information along the spatial dimension.
Specifically, the $A(x,y,\lambda)$  of AEM-P encodes the unit shift of the mask upwards layer by layer in the spectral dimension.
\begin{equation}
	A(x,y,\lambda) = Mask_{P}(x,y,\theta_{mask_p}) \cdot Dispersive(\lambda),
\end{equation}	
where, the $Mask_{P}$ denotes the spatial dimensional encoding mask, the $\theta_{mask_p}$ is a learnable parameters, and the $Dispersive(\lambda)$ represents the dispersion operation.

The imaging process of AEM-P can be written based on Eq.~(\ref{eq:uem}) as follows:
\begin{equation}
	I_{rgb} = \int W(\lambda) \cdot (A(x,y,\lambda)\cdot I(x,y,\lambda) ) d\lambda.
\label{aemp_imaging}
\end{equation}	


\begin{figure}[!t]
\centering
\subfloat[Optical encoding propagation of SD-CASSI.]{\includegraphics[width=3in]{Figure/sdcassi_paint.pdf}}
\label{sdcassi_paint}

\subfloat[Encoding parameterization (height map) and the optical path of the rotationally symmetric DOE (R. S. DOE).]{\includegraphics[width=3in]{Figure/DOE_propogation.pdf}}
\label{fig_PSFSHOW}

\subfloat[Response curve and optical path of wavelength encoding.]{\includegraphics[width=3in]{Figure/filter_sensor.pdf}}
\label{fig_DOE_propogation}

\caption{Optical Path of the UEMs.}
\label{fig_uempaint}
\end{figure}


% \begin{figure}[!t]
% \centering
% \subfloat[Height Map]{\includegraphics[width=1.2in]{Figure/rotadoe_paint.png}}
% \label{rotadoe_paint}
% \hfil
% \subfloat[Optical Path]{\includegraphics[width=2in]{Figure/DOE_propogation.png}}
% \label{fig_DOE_propogation}

% \caption{Encoding parameterization (height map) and the optical path of the rotationally symmetric DOE (R. S. DOE).}
% \label{fig_PSFSHOW}
% \end{figure}


\noindent {\bf{Physical Phase Encoding Model.}} 

The PEM-P utilizes the height map of the DOE or the structure of the metasurface to produce a phase delay as modulation. 
Following the common settings, we model PEM-P based on a rotationally symmetric DOE, as shown in Figure~\ref{fig_uempaint}(b), which uses a one-dimensional parameter to represent the entire DOE height map. This parameterization reduces both the number of learnable parameters and manufacturing complexity.
The height map $H(x,y)$ of a rotationally symmetric DOE can be represented as follows:
\begin{equation}
	H(x,y) = H_{P}(x,y,\theta_{height map}),
\end{equation}	
where the $H_{P}$ is the height map, and the $\theta_{height map}$ is a one-dimensional learnable parameter.


The PSF $P(x,y,\lambda)$ can be derivated from the height map $H(x,y)$ according to diffraction law. For the detailed derivation, please refer to the supplement. 
Then, the imaging process of PEM-P can be written based on Eq.~(\ref{eq:uem}):
\begin{equation}
	I_{rgb} = \int W(\lambda) \cdot (P(x,y,\lambda) \ast I(x,y,\lambda)) d\lambda.
\label{pemp_imaging}
\end{equation}	


\noindent {\bf{Physical Wavelength Encoding Model.}}

The WEM-P fixes all other system components and replaces the spectral response curve with different options to select the best-performing one, in cases where a non-learnable spectral response curve is used. 
\begin{equation}
	W(\lambda) = \{w_i\vert w_i \in \mathbf{W}, w_i\ is\ the \ most \ suited\},
\end{equation}
where the $w_1,w_2,w_2,... \in \mathbf{W}$ represents a fixed response function dataset.

The imaging process of WEM-P can be written from Eq.~(\ref{eq:uem}) by eliminating unused terms:
\begin{equation}
	I_{rgb} = \int W(\lambda) \cdot I(x,y,\lambda) d\lambda.
\label{wemp_imaging}
\end{equation}

\subsection{Ideal Model}
We then introduce the ideal UEMs, AEM-I, PEM-I, and WEM-I, which are free from any physical constraint in the physical UEMs.

\noindent {\bf{Ideal Amplitude Encoding Model.}} 
Compared to AEM-P, we design the AEM-I using floating point encoding to encode spatial and spectral dimensional encoding mask $A_{I}(x,y,\lambda)$.

The imaging model of AEM-I is obtained by replacing $A(x,y,\lambda)$ in Eq.~(\ref{aemp_imaging}) with $A_{I}(x,y,\lambda)$.
\begin{equation}
	A_{I}(x,y,\lambda) = Mask_{I}(x,y,\lambda,\theta_{mask}),
\end{equation}	
where the $Mask_{I}$ is the spatial and spectral dimensional encoding mask, the $\theta_{mask}$ is a learnable parameters. 


\noindent {\bf{Ideal Phase Encoding Model.}} 
% The PSF in the phase encoding ideal model (PEM-I) is determined by the physical characteristics of the DOE and Metasurface. 
We encode the PSF $P_I(x,y,\lambda)$ directly for the PEM-I without considering the structure of the DOE of PEM-P.
%the physical constraints of the PEM-P's diffractive elements.
The imaging model of PEM-I is obtained by replacing $P(x,y,\lambda)$ in Eq.~(\ref{pemp_imaging}) with $P_I(x,y,\lambda)$.
\begin{equation}
	P_I(x,y,\lambda) = PSF_I(x,y,\lambda,\theta_{psf}),
\end{equation}	
where the $PSF_{I}$ is the spatial and spectral dimensional encoding psf, the $\theta_{psf}$ is a learnable parameters. 


\noindent {\bf{Ideal Wavelength Encoding Model.}} 
% The advancement in filter surface coating technology has led to the development of sensors with customizable spectral response curves, allowing for greater flexibility in designing computational spectral imaging systems. 
Although it is possible to customize the spectral curve as required in filter surface coating technology, the constraints of the filter material properties still need to be considered when designing the system. 
Our WEM-I directly encodes the spectral profile without regard to the constraints of WEM-P. 
The imaging model of PEM-I is obtained by replacing $W(x,y,\lambda)$ in Eq.~(\ref{wemp_imaging}) with $W_I(x,y,\lambda)$.
\begin{equation}
	W_{I}(\lambda) = Response_{I}(\lambda,\theta_{response}),
\end{equation}
where the $Response_{I}$ is the encoding response function, and the $\theta_{response}$ is a learnable parameters.


\section{Joint Optimization}
In this section, we introduce the decoding models we use and the optimization objective in the joint optimization framework for the comparative study.

\noindent {\bf{Decoding Model.}} 

Since we are mainly exploring the performance of several encoding models rather than the decoding models, we employ a simple CNN~\cite{lecun1998gradient,lee2017going,maffei2019single}, a variant of the popular U-Net~\cite{ronneberger2015u,miao2019net}, Res-U-Net~\cite{zhang2018road,gurrola2021residual} and Unfolding-Net~\cite{dong2018denoising,zhang2020deep,zhang2020amp,sun2021deep,zhang2021plug,zhang2022herosnet,cai2022degradation}, as reconstruction networks. For the detailed network structure, please refer to the supplement.

\begin{figure*}[!t]
\centering
\includegraphics[width=6.5in]{Figure/framework.pdf}
\caption{Joint encoder-decoder optimization framework optimizes the UEM and the decoding model toward the same objective.}
\label{fig_joint_optimization_framework}
\end{figure*}



\noindent {\bf{Joint Optimization Framework.}} %待修改
We combine the UEM with the decoding model to compose a joint encoder-decoder optimization framework.

In the UEM, scene light gets amplitude modulation $f_A(I,\theta_{A})$, gets phase modulated $f_P(I,\theta_{P})$, passes through the filter and the sensor to obtain a spectral dimensional blending $f_W(I,\theta_{W})$. We can describe the overall imaging process as follow:
\begin{equation}
	I_{rgb} = f_A(f_P(f_W(I,\theta_{A}),\theta_{P}),\theta_{W}),
\end{equation}		
where $\theta_{A}$,$\theta_{P}$, and $\theta_{W}$ are learnable parameters for the AEM, the PEM, and the WEM. For each system only optimizes one parameter, e.g. for AEM systems only $\theta_{A}$ is optimized. After that, the decoding model reconstructs the spectral images from the RGB measurement $I_{rgb}$, and this process can be written as:
\begin{equation}
	\tilde{I} = f_{D}(I_{rgb},\theta_{D}),
\end{equation}	
where the $\theta_{D}$ is the learnable parameter of the decoding model.

Then, the optimization objective of the UEM is to find a set of $\theta_{A},\theta_{P},\theta_{W},\theta_{D}$ that minimizes the mean absolute error (MAE) loss between the reconstructed spectral images and the ground truth:
\begin{equation}
\theta_{A},\theta_{P},\theta_{W},\theta_{D} = \mathop{\arg\min}_{\theta_{A},\theta_{P},\theta_{W},\theta_{D}}{\sum \Vert\tilde{I} - I\Vert}.
 % (\tilde{I},I,\theta_{A},\theta_{P},\theta_{W},\theta_{D})}} = {{\underset{{\theta_{A},\theta_{P},\theta_{W},\theta_{D}}}{\arg\min}} {\sum ||\tilde{I},I||}},  
\end{equation}

Since each stage of the UEM is differentiable, we can solve this problem using the first-order gradient-based optimization methods. When we cast the UEM to a specific encoding model, the irrelevant parameter will be eliminated. That is, we only optimize $\theta_{A},\theta_{D}$ for AEMs, $\theta_{P},\theta_{D}$ for PEMs, and $\theta_{W},\theta_{D}$ for WEMs.

Finally, we combine the UEM, decoding model, and optimization objective together to build a joint encoder-decoder optimization framework, as shown in Figure~\ref{fig_joint_optimization_framework}.



==> sec/4_experiment.tex <==
\section{Experiments and Analysis}

%UEM的具体实验设置
\subsection{Experimental Setup}
%

In our experiments, we predominantly employ the Sim-Conv-Net as the decoding model. We also conduct additional experiments using Res-U-Net and Unfolding-Net to compare the choice of decoding model.
We adopt the nearest neighbor interpolation from RGB images to the spectral image as the naive baseline of spectral imaging.
The details of the decoding model are described in suplement.
%, which is demonstrated in Figure~\ref{baseline}


% \begin{figure}[!t]
% \centering
% {\includegraphics[width=3.2in]{Figure/baseline.png}}
% \caption{Baseline: nearest neighbor interpolation from the RGB image into the spectral image.}
% \label{baseline}
% \end{figure}

Our joint encoder-decoder optimization framework is evaluated on four datasets, ICVL\cite{arad2016sparse}, Harvard~\cite{chakrabarti2011statistics}, CAVE~\cite{CAVE_0293}, and KAIST~\cite{DeepCASSI:SIGA:2017}, and cross-validated. Among them, the ICVL dataset is the main one, which we divided into 167 images for training, 17 for validation, and 17 for testing. All images are cropped to 512 × 512 patches. To demonstrate the validity of the dataset, we also performed additional validation experiments on ICVL, which are shown in the supplement.

% Our joint encoder-decoder optimization framework is primarily evaluated on the ICVL~\cite{arad2016sparse} dataset, we split it into 167 images for training, 17 for validation, and 17 for testing. All images are cropped to 512 × 512 patches. 
The response curve of the FLIR BFS\_U3\_04S2C\_C camera is used in experiments where the response is fixed (AEM, PEM and WEM-P). 
For evaluation metrics, we adopt PSNR, PSNR-SI, SAM, and ERGAS as evaluation metrics, where the PSNR-SI is the average PSNR of each channel of the spectral image, and the max intensity in this PSNR calculation is set to the channel maximum of the corresponding ground truth instead of the maximum possible pixel value.

 
%待调整
\begin{table*}[!t]
    \centering
    \caption{Spectral imaging performance of systems using UEMs on different datasets, with the best results in bold.}
    \label{table_simconv}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{c|c|cccc|c|cccc}
    \hline
        ~ & \multicolumn{5}{c|}{\textbf{Physical Model}}& \multicolumn{5}{c}{\textbf{Ideal Model}} \\ \hline
        \textbf{Datasets} & \textbf{Encoding Model} & \textbf{PSNR$\uparrow$} & \textbf{PSNR-SI$\uparrow$} & \textbf{SAM$\downarrow$} & \textbf{ERGAS$\downarrow$} & \textbf{Encoding Model} & \textbf{PSNR$\uparrow$} & \textbf{PSNR-SI$\uparrow$} & \textbf{SAM$\downarrow$} & \textbf{ERGAS$\downarrow$}  \\ \hline
        \multirow{2}*{\textbf{ICVL}} & \textbf{WEM-P} & 44.96 & 38.81 & 0.0399 & 6.23 & \textbf{WEM-I} & \textbf{45.25} & 38.51 & \textbf{0.0328} & \textbf{5.23}  \\ 
        ~ & \textbf{AEM-P} & 40.21 & 32.66 & 0.0491 & 8.96 & \textbf{AEM-I} & 45.08 & \textbf{38.95} & 0.0405 & 6.24  \\ 
        \multirow{2}*{(training \& testing)} & \textbf{PEM-P} & 33.75 & 26.02 & 0.0655 & 16.62 & \textbf{PEM-I} & 44.9 & 38.68 & 0.0398 & 6.28  \\ 
        ~ & \textbf{Baseline} & 32.21 & 28.98 & 0.1342 & 33.3 &    &   &   &   &   \\ \hline
        \multirow{2}*{\textbf{Harvard}} & \textbf{WEM-P} & 38.72 & 36.91 & 0.07538 & 8.01 & \textbf{WEM-I} & \textbf{39.9} & 36.31 & \textbf{0.05152} & 8.09  \\ 
        ~ & \textbf{AEM-P} & 32.7 & 30.01 & 0.0852 & 14.04 & \textbf{AEM-I} & 38.84 & \textbf{36.88} & 0.07513 & \textbf{7.97}  \\ 
        \multirow{2}*{(training \& testing)} & \textbf{PEM-P} & 27.24 & 24.42 & 0.10196 & 25.17 & \textbf{PEM-I} & 38.71 & \textbf{36.88} & 0.07561 & 8.12  \\ 
        ~ & \textbf{Baseline} & 26.28 & 24.87 & 0.21845 & 143.05 &    &   &   &   &   \\ \hline
        \multirow{2}*{\textbf{CAVE}} & \textbf{WEM-P} & 36.02 & 37.57 & 0.1961 & 18.38 & \textbf{WEM-I} & \textbf{37.65} & 37.98 & 0.1682 & 17.48  \\ 
        ~ & \textbf{AEM-P} & 33.13 & 33.13 & 0.2193 & 26.11 & \textbf{AEM-I} & 36.96 & \textbf{38.00} & \textbf{0.1590} & \textbf{16.85}   \\ 
        \multirow{2}*{(training \& testing)} & \textbf{PEM-P} & 28.99 & 28.76 & 0.2974 & 48.23 & \textbf{PEM-I} & 35.77 & 37.55 & 0.1894 & 18.77  \\ 
        ~ & \textbf{Baseline} & 29.50 & 30.36 & 0.3906 & 41.74 &    &   &   &   &   \\  \hline
        \multirow{2}*{\textbf{CAVE} (training),} & \textbf{WEM-P} & 32.02 & 33.58 & 0.4819 & 36.82 & \textbf{WEM-I} & 33.04 & 31.93 & 0.4363 & 43.45  \\ 
        ~ & \textbf{AEM-P} & 32.21 & 33.69 & 0.4707 & 36.22 & \textbf{AEM-I} & \textbf{33.30} & \textbf{34.42} & \textbf{0.3679} & \textbf{31.82}  \\ 
        \multirow{2}*{\textbf{KAIST} (testing)} & \textbf{PEM-P} & 28.39 & 26.20 & 0.4909 & 70.45 & \textbf{PEM-I} & 30.68 & 29.60 & 0.4541 & 48.82  \\ 
        ~ & \textbf{Baseline} & 30.78 & 31.06 & 0.6339 & 46.47 &    &   &   &   &   \\ \hline
    \end{tabular}}
\end{table*}
% \begin{table*}[!t]
%     \centering
%     \caption{Spectral imaging performance of systems using UEMs on different datasets, with the best results in bold.}
%     \label{table_simconv}
%     \resizebox{\linewidth}{!}{
%     \begin{tabular}{c|c|cccc|c|cccc}
%     \hline
%         ~ & \multicolumn{5}{c|}{\textbf{Physical Model}}& \multicolumn{5}{c}{\textbf{Ideal Model}} \\ \hline
%         \textbf{Datasets} & \textbf{Encoding Model} & \textbf{PSNR$\uparrow$} & \textbf{PSNR-SI$\uparrow$} & \textbf{SAM$\downarrow$} & \textbf{ERGAS$\downarrow$} & \textbf{Encoding Model} & \textbf{PSNR$\uparrow$} & \textbf{PSNR-SI$\uparrow$} & \textbf{SAM$\downarrow$} & \textbf{ERGAS$\downarrow$}  \\ \hline
%         \multirow{2}*{\textbf{ICVL}} & \textbf{WEM-P} & 44.96 & 38.81 & 0.0399 & 6.23 & \textbf{WEM-I} & \textbf{45.25} & 38.51 & \textbf{0.0328} & \textbf{5.23}  \\ 
%         ~ & \textbf{AEM-P} & 40.21 & 32.66 & 0.0491 & 8.96 & \textbf{AEM-I} & 45.08 & \textbf{38.95} & 0.0405 & 6.24  \\ 
%         \multirow{2}*{(training \& testing)} & \textbf{PEM-P} & 33.75 & 26.02 & 0.0655 & 16.62 & \textbf{PEM-I} & 44.9 & 38.68 & 0.0398 & 6.28  \\ 
%         ~ & \textbf{Baseline} & 32.21 & 28.98 & 0.1342 & 33.3 &   &   &   &   &    \\ \hline
%         \multirow{2}*{\textbf{Harvard}} & \textbf{WEM-P} & 38.72 & 36.91 & 0.0754 & 8.01 & \textbf{WEM-I} & \textbf{39.9} & 36.31 & \textbf{0.0515} & \textbf{7.97}  \\ 
%         ~ & \textbf{AEM-P} & 32.7 & 30.01 & 0.0852 & 14.04 & \textbf{AEM-I} & 38.84 & \textbf{36.88} & 0.0751 & 8.09  \\ 
%         \multirow{2}*{(training \& testing)} & \textbf{PEM-P} & 27.24 & 24.42 & 0.1019 & 25.17 & \textbf{PEM-I} & 38.71 & \textbf{36.88} & 0.0756 & 8.12  \\ 
%         ~ & \textbf{Baseline} & 26.28 & 24.87 & 0.2184 & 143.05 &   &   &   &   &    \\ \hline
%         \multirow{2}*{\textbf{CAVE}} & \textbf{WEM-P} & 36.02 & 37.57 & 0.1961 & 18.38 & \textbf{WEM-I} & \textbf{37.65} & 37.98 & \textbf{0.1590} & \textbf{16.85}  \\ 
%         ~ & \textbf{AEM-P} & 33.13 & 33.13 & 0.2193 & 26.11 & \textbf{AEM-I} & 36.96 & \textbf{38.00} & 0.1682 & 17.48   \\ 
%         \multirow{2}*{(training \& testing)} & \textbf{PEM-P} & 28.99 & 28.76 & 0.2974 & 48.23 & \textbf{PEM-I} & 35.77 & 37.55 & 0.1894 & 18.77  \\ 
%         ~ & \textbf{Baseline} & 29.50 & 30.36 & 0.3906 & 41.74 &   &   &   &   &    \\  \hline
%         \multirow{2}*{\textbf{CAVE} (training),} & \textbf{WEM-P} & 32.21 & 33.69 & 0.4707 & 36.22 & \textbf{WEM-I} & \textbf{33.30} & \textbf{34.42} & \textbf{0.3679} & \textbf{31.82}  \\ 
%         ~ & \textbf{AEM-P} & 32.02 & 33.58 & 0.4819 & 36.82 & \textbf{AEM-I} & 33.04 & 31.93 & 0.4363 & 43.45  \\ 
%         \multirow{2}*{\textbf{KAIST} (testing)} & \textbf{PEM-P} & 28.39 & 26.20 & 0.4909 & 70.45 & \textbf{PEM-I} & 30.68 & 29.60 & 0.4541 & 48.82  \\ 
%         ~ & \textbf{Baseline} & 30.78 & 31.06 & 0.6339 & 46.47 &   &   &   &   &    \\ \hline
%     \end{tabular}}
% \end{table*}

% \begin{table*}[!t]
%     \centering
%     \caption{Spectral imaging performance of systems using UEMs on different datasets, with the best results in bold.}
%     \label{table_simconv}
%     \resizebox{\linewidth}{!}{
%     \begin{tabular}{c|c|cccc|c|cccc}
%     \hline
%         ~ & \multicolumn{5}{c|}{\textbf{Physical Model}}& \multicolumn{5}{c}{\textbf{Ideal Model}} \\ \hline
%         \textbf{Datasets} & \textbf{Encoding Model} & \textbf{PSNR$\uparrow$} & \textbf{PSNR-SI$\uparrow$} & \textbf{SAM$\downarrow$} & \textbf{ERGAS$\downarrow$} & \textbf{Encoding Model} & \textbf{PSNR$\uparrow$} & \textbf{PSNR-SI$\uparrow$} & \textbf{SAM$\downarrow$} & \textbf{ERGAS$\downarrow$}  \\ \hline
%         \multirow{2}*{\textbf{ICVL}} & \textbf{WEM-P} & 44.96 & 38.81 & 0.0399 & 6.23 & \textbf{WEM-I} & \textbf{45.25} & 38.51 & \textbf{0.0328} & \textbf{5.23}  \\ 
%         ~ & \textbf{AEM-P} & 40.21 & 32.66 & 0.0491 & 8.96 & \textbf{AEM-I} & 45.08 & \textbf{38.95} & 0.0405 & 6.24  \\ 
%         \multirow{2}*{(training \& testing)} & \textbf{PEM-P} & 33.75 & 26.02 & 0.0655 & 16.62 & \textbf{PEM-I} & 44.9 & 38.68 & 0.0398 & 6.28  \\ 
%         ~ & \textbf{Baseline} & 32.21 & 28.98 & 0.1342 & 33.3 & \textbf{N/A} & - & - & - & -  \\ \hline
%         \multirow{2}*{\textbf{Harvard}} & \textbf{WEM-P} & 38.72 & 36.91 & 0.07538 & 8.01 & \textbf{WEM-I} & \textbf{39.9} & 36.31 & \textbf{0.05152} & 8.09  \\ 
%         ~ & \textbf{AEM-P} & 32.7 & 30.01 & 0.0852 & 14.04 & \textbf{AEM-I} & 38.84 & \textbf{36.88} & 0.07513 & \textbf{7.97}  \\ 
%         \multirow{2}*{(training \& testing)} & \textbf{PEM-P} & 27.24 & 24.42 & 0.10196 & 25.17 & \textbf{PEM-I} & 38.71 & \textbf{36.88} & 0.07561 & 8.12  \\ 
%         ~ & \textbf{Baseline} & 26.28 & 24.87 & 0.21845 & 143.05 & \textbf{N/A} & - & - & - & -  \\ \hline
%         \multirow{2}*{\textbf{CAVE}} & \textbf{WEM-P} & 36.02 & 37.57 & 0.1961 & 18.38 & \textbf{WEM-I} & \textbf{37.65} & 37.98 & 0.1682 & 17.48  \\ 
%         ~ & \textbf{AEM-P} & 33.13 & 33.13 & 0.2193 & 26.11 & \textbf{AEM-I} & 36.96 & \textbf{38.00} & \textbf{0.1590} & \textbf{16.85}   \\ 
%         \multirow{2}*{(training \& testing)} & \textbf{PEM-P} & 28.99 & 28.76 & 0.2974 & 48.23 & \textbf{PEM-I} & 35.77 & 37.55 & 0.1894 & 18.77  \\ 
%         ~ & \textbf{Baseline} & 29.50 & 30.36 & 0.3906 & 41.74 & \textbf{N/A} & - & - & - & -  \\  \hline
%         \multirow{2}*{\textbf{CAVE} (training),} & \textbf{WEM-P} & 32.02 & 33.58 & 0.4819 & 36.82 & \textbf{WEM-I} & 33.04 & 31.93 & 0.4363 & 43.45  \\ 
%         ~ & \textbf{AEM-P} & 32.21 & 33.69 & 0.4707 & 36.22 & \textbf{AEM-I} & \textbf{33.30} & \textbf{34.42} & \textbf{0.3679} & \textbf{31.82}  \\ 
%         \multirow{2}*{\textbf{KAIST} (testing)} & \textbf{PEM-P} & 28.39 & 26.20 & 0.4909 & 70.45 & \textbf{PEM-I} & 30.68 & 29.60 & 0.4541 & 48.82  \\ 
%         ~ & \textbf{Baseline} & 30.78 & 31.06 & 0.6339 & 46.47 & \textbf{N/A} & - & - & - & -  \\ \hline
%     \end{tabular}}
% \end{table*}

\begin{figure}[!t]

\centering
\subfloat[GT]{\begin{overpic}[width=0.7in]{Figure/GT.png}
\end{overpic}}
\label{GT}
\subfloat[WEM-I]{\begin{overpic}[width=0.7in]{Figure/reconstructed_coded_sensor.png}
\end{overpic}}
\label{reconstructed_coded_sensor}
\subfloat[AEM-I]{\begin{overpic}[width=0.7in]{Figure/reconstructed_3dcassi.png}
\end{overpic}}
\label{reconstructed_3dcassi} 
\subfloat[PEM-I]{\begin{overpic}[width=0.7in]{Figure/reconstructed_freepsf.png}
\end{overpic}}
\label{reconstructed_freepsf} 

\subfloat[Baseline]{\begin{overpic}[width=0.7in]{Figure/reconstructed_baseline.png}
\end{overpic}}
\label{reconstructed_baseline} 
\subfloat[WEM-P]{\begin{overpic}[width=0.7in]{Figure/reconstructed_nopsf.png}
\end{overpic}}
\label{reconstructed_nopsf}
\subfloat[AEM-P]{\begin{overpic}[width=0.7in]{Figure/reconstructed_sdcassi.png}
\end{overpic}}
\label{reconstructed_sdcassi}
\subfloat[PEM-P]{\begin{overpic}[width=0.7in]{Figure/reconstructed_rotadoe.png}
\end{overpic}}

\label{reconstructed_rotadoe}

\caption{Visual comparison of reconstruction images.}
\label{fig_reconsted_result}
\end{figure}


\begin{figure}[!t]
\centering
{\includegraphics[width=3.2in]{Figure/red_curve.pdf}}
\caption{Spectral curve comparison at a single sampling point.}
\label{fig_red_curve}
\end{figure}

% \begin{figure}[!t]
% \centering
% {\includegraphics[width=0.5in]{Figure/red_doll.png}}
% \label{red_doll}
% {\includegraphics[width=2.5in]{Figure/red_curve.pdf}}
% \label{red_curve}
% \caption{Spectral curve comparison at a single sampling point.}
% \label{fig_red_curve}
% \end{figure}

\subsection{Results}

\noindent {\bf{Comparative Experiments on Different Datasets.}} 
The Table~\ref{table_simconv} shows a comparison of the spectral imaging performance of the system consisting of UEMs and Sim-Conv-Net on different datasets. The imaging effects of the various sub-models of the UEM show similar regularity across experiments with different datasets.
Among the physical models, the WEM-P performs the best, followed by the AEM-P, and the PEM-P is the worst.
Similarly, the WEM-I also has the best imaging results among the ideal models. 
Since the WEM-P already has the best performance in physical models, the improvement brought by its ideal model WEM-I is relatively small. 
Conversely, the AEM-P and the PEM-P exhibit greater potential for enhancement relative to their corresponding ideal models. 

In addition, to evaluate the generalizability of our systems, we also train our models using the CAVE dataset and test them on the KAIST dataset. In this experiment, only the overlapped bands of CAVE and KAIST are used for training and test
It is interesting that the AEMs seem to have the best generalizability, while the WEM-P and the PEM-I trained on the CAVE dataset show significant performance drops when testing with the KAIST dataset. 
% The ``ICVL" row of Table~\ref{table_simconv} shows a comparison of the spectral imaging performance of the system consisting of UEMs and Sim-Conv-Net on ICVL.
% Among the physical models, the WEM-P performs the best, followed by the AEM-P, and the PEM-P is the worst.
% Similarly, the WEM-I also has the best imaging results among the ideal models. 
% Since the WEM-P already has the best performance in physical models, the improvement brought by its ideal model WEM-I is relatively small. 
% Conversely, the AEM-P and the PEM-P exhibit greater potential for enhancement relative to their corresponding ideal models. % The evaluation metrics show 



The RGB visualizations of reconstructed spectral images of all the models are presented in Figure~\ref{fig_reconsted_result}. Although the WEM-I outperforms the other models in numeric results, it still has slight color inaccuracies in some cases, for example, an overall orange shift shown in Figure~\ref{fig_reconsted_result} (b). This shift may be attributed to the presence of negative values in the response curve of the free encoding. 
The PEM-P exhibits poorer reconstruction performance for both color and image detail, which is consistent with the numeric metrics.

Besides numerical and visual evaluation, we randomly choose an area in the visualized scene and extract its spectral curve to compare the spectral accuracy of each model, as illustrated in Figure~\ref{fig_red_curve}. 
The results show that the curve of the WEM-I matches the ground truth best, while the PEM-P is even less accurate than the baseline. The other physical and idea models exhibit a relatively close curve around the ground truth, which is also consistent with the numeric metrics.



% \noindent {\bf{Comparative Experiments on Other Datasets.}} 
% We perform additional experiments on the CAVE~\cite{CAVE_0293} and Harvard~\cite{chakrabarti2011statistics} datasets. 
% As shown in the ``CAVE" and ``Harvard" rows of Table~\ref{table_simconv}, we observe that the results are similar to the results on ICVL, and the WEMs are still the generally best model.

% In addition, to evaluate the generalizability of our systems, we also train our models using the CAVE dataset and test them on the KAIST~\cite{DeepCASSI:SIGA:2017} dataset. In this experiment, only the overlapped bands of CAVE and KAIST are used for training and test
% The results are shown in the ``CAVE, KAIST" row of Table~\ref{table_simconv}.
% It is interesting that the AEMs seem to have the best generalizability, while the WEM-P and the PEM-I trained on the CAVE dataset show significant performance drops when testing with the KAIST dataset. 


\begin{table}[!t]
  \centering
  \caption{Using Res-U-Net as the decoding model, with the best results in bold and the next best results underlined in each column.}
  \label{table_resunet7}
  \resizebox{\linewidth}{!}
  {\begin{tabular}{ccccc}
  \hline
    \textbf{Encoding Model} & \textbf{PSNR$\uparrow$} & \textbf{PSNR-SI$\uparrow$} & \textbf{SAM$\downarrow$} & \textbf{ERGAS$\downarrow$} \\ \hline
    \textbf{WEM-P} & 38.62 & 32.00 & \underline{0.0373} & 8.07 \\ 
    \textbf{AEM-P} & 36.72 & 29.53 & 0.0422 & 10.39 \\
    \textbf{PEM-P} & 34.87 & 28.10 & 0.0654 & 13.08 \\ 
    \textbf{Baseline} & 32.21 & 28.98 & 0.1342 & 33.30 \\ \hline
    \textbf{WEM-I} & \textbf{40.54} & \textbf{33.96} & \textbf{0.0359} & \textbf{6.73} \\ 
    \textbf{AEM-I} & \underline{39.28} & \underline{32.80} & 0.0395 & \underline{7.51} \\ 
    \textbf{PEM-I} & 38.57 & 31.83 & 0.0386 & 8.15 \\ 
     \hline
  \end{tabular}}
\end{table}

\noindent {\bf{Experiments on Different Decoding Model.}} 
In this experiment, we replaced the decoding model Sim-Conv-Net with a Res-U-Net, and the results are shown in Table~\ref{table_resunet7}. Although increasing the depth and complexity of the network should have led to better image reconstruction, we observed lower metrics when using Res-U-Net in our end-to-end optimization experiments. With the exception of WEM-I, the tables suggest that metrics sensitive to spatial differences, such as PSNR, tend to be higher in models utilizing the Sim-Conv-Net. In contrast, metrics sensitive to spectral errors, such as SAM, are generally better in models using Res-U-Net as the decoding model. Additionally, we noticed that only the PEM-P showed an improvement in imaging performance when using Res-U-Net compared to the Sim-Conv-Net.

Training a very large network structure in an end-to-end optimized computational spectral imaging system may prove to be challenging. Therefore, we suggest that simple convolutional neural networks with only a few layers may suffice to achieve satisfactory results. We also recommend that simpler optical encoding processes are better suited for simple networks, whereas deeper networks should be chosen for more complex encoding models.


\begin{figure*}[!t]
\centering
\subfloat[Sim-Conv-Net, channel 6-11]{\includegraphics[width=3.25in]{Figure/freepsf_sim_6-11.png}}
\label{fig_freepsf_sim_6-11}
\hfil
\subfloat[Sim-Conv-Net, channel 18-23]{\includegraphics[width=3.25in]{Figure/freepsf_sim_18-23.png}}
\label{fig_freepsf_sim_18-23}

\subfloat[Res-U-Net (depth=7), channel 6-11]{\includegraphics[width=3.25in]{Figure/freepsf_res7_6-11.png}}
\label{fig_freepsf_res7_6-11}
\hfil
\subfloat[Res-U-Net (depth=7), channel 18-23]{\includegraphics[width=3.25in]{Figure/freepsf_res7_18-23.png}}
\label{fig_freepsf_res7_18-23}

\caption{Visual comparison of the PSFs of PEM-I using different decoding networks. The PSF energy of the Sim-Conv-Net is more convergent at the center and the PSF pattern is differentiated between channels. The PSFs of the Res-U-Net are more diffuse and have no obvious regularity.}
\label{fig_freepsf}
\end{figure*}

We also design unfolding network as the decoding model to further improve the performance of ideal model, and the results are shown in Table~\ref{table_unfoldingnet}. 

\begin{table}[!ht]
    \centering
    \caption{Using unfolding networks as the decoding model.}
  \label{table_unfoldingnet}
  \resizebox{\linewidth}{!}{
    \begin{tabular}{ccccccc}
    \hline
        \textbf{Encoding Model} & \textbf{PSNR$\uparrow$} & \textbf{PSNR-SI$\uparrow$} & \textbf{SAM$\downarrow$} & \textbf{ERGAS$\downarrow$} \\ \hline
        WEM-I & \textbf{46.43} & \textbf{40.86} & \textbf{3.69} & \textbf{0.0257} \\ 
        AEM-I & 46.33 & 40.30 & 3.71 & 0.0280 \\ 
        PEM-I & 45.94 & 40.53 & 3.84 & 0.0286 \\ \hline
    \end{tabular}}
\end{table}



% \subsection{Image Segmentation}
\noindent {\bf{Experiments on Image Segmentation.}} 
In real-world applications, spectral images captured by spectral imaging systems are often utilized for various high-level tasks. Thus, evaluating the imaging performance of these spectral imaging systems may be insufficient, and how much can they assist the perceptual tasks is worth to be explored. Thus, we select spectral image segmentation as the target perceptual task to evaluate the performance of spectral imaging systems on high-level tasks. 
For this purpose, we employ a Res-U-Net as the segmentation network and evaluate the segmentation performance on the LIB-HSI dataset~\cite{habili2023hyperspectral}.

We acquired spectral images from each spectral imaging system and then input them into the segmentation network for evaluation. Table~\ref{table_segmentation} shows the comparison of the segmentation accuracy of previously discussed UEMs accompanied with the same trained segmentation network. Te segmentation visualization results are shown in Figure~\ref{fig_seg_result}. 
Despite the AEM-P outperforming the PEM-P in spectral imaging, it performs worse than the PEM-P on the segmentation task, indicating the absence of a positive correlation between the low-level imaging and high-level segmentation performance. 
We conclude that while phase encoding presents greater difficulty in decoding overlapping information than amplitude and wavelength encoding, it may retain more comprehensive semantic information about the image, thus promoting its image segmentation performance.


\begin{table}[!t]
  \centering
  \caption{Comparison of the segmentation quality of all systems, with the best results in bold and the next best results underlined.}
  \label{table_segmentation}
  \resizebox{\linewidth}{!}{
  \begin{tabular}{cc|cc}
  \hline
   \multicolumn{2}{c|}{\textbf{Physical Model}}& \multicolumn{2}{c}{\textbf{Ideal Model}} \\ \hline
    \textbf{Encoding Model} & \textbf{Accuracy$\uparrow$} & \textbf{Encoding Model} & \textbf{Accuracy$\uparrow$} \\ \hline
    % \textbf{No Imaging} & \textbf{0.61541} &  \\ 
    \textbf{WEM-P} & 0.5218 & \textbf{WEM-I} & \underline{0.5221}\\ 
    \textbf{AEM-P} & 0.4151 & \textbf{AEM-I} & \textbf{0.5234}\\ 
    \textbf{PEM-P} & 0.4479 & \textbf{PEM-I} & 0.5128 \\
    \textbf{Baseline} & 0.3223 &   &   \\\hline
  \end{tabular}}
\end{table}

% \begin{table}[!t]
%   \centering
%   \caption{Comparison of the segmentation quality of all systems, with the best results in bold and the next best results underlined.}
%   \label{table_segmentation}
%   \resizebox{\linewidth}{!}{
%   \begin{tabular}{cc|cc}
%   \hline
%    \multicolumn{2}{c|}{\textbf{Physical Model}}& \multicolumn{2}{c}{\textbf{Ideal Model}} \\ \hline
%     \textbf{Encoding Model} & \textbf{Accuracy$\uparrow$} & \textbf{Encoding Model} & \textbf{Accuracy$\uparrow$} \\ \hline
%     % \textbf{No Imaging} & \textbf{0.61541} &  \\ 
%     \textbf{WEM-P} & 0.5218 & \textbf{WEM-I} & \underline{0.5221}\\ 
%     \textbf{AEM-P} & 0.4151 & \textbf{AEM-I} & \textbf{0.5234}\\ 
%     \textbf{PEM-P} & 0.4479 & \textbf{PEM-I} & 0.5128 \\
%     \textbf{Baseline} & 0.3223 & N/A & - \\\hline
%   \end{tabular}}
% \end{table}

\begin{figure}[!t]

\centering
\subfloat[RGB Image]{\includegraphics[width=1in,angle=-90]{Figure/seg_image.png}}
\label{seg_image}
\subfloat[GT]{\includegraphics[width=1in,angle=-90]{Figure/seg_gt.png}}
\label{seg_GT}
\subfloat[Baseline]{\includegraphics[width=1in,angle=-90]{Figure/seg_baseline.png}}
\label{seg_baseline}


\subfloat[WEM-I]{\includegraphics[width=1in,angle=-90]{Figure/seg_wemi.png}}
\label{seg_wemi}
\subfloat[AEM-I]{\includegraphics[width=1in,angle=-90]{Figure/seg_aemi.png}}
\label{seg_aemi}
\subfloat[PEM-I]{\includegraphics[width=1in,angle=-90]{Figure/seg_pemi.png}}
\label{seg_pemi}

\subfloat[WEM-P]{\includegraphics[width=1in,angle=-90]{Figure/seg_wemp.png}}
\label{seg_wemp}
\subfloat[AEM-P]{\includegraphics[width=1in,angle=-90]{Figure/seg_aemp.png}}
\label{seg_aemp}
\subfloat[PEM-P]{\includegraphics[width=1in,angle=-90]{Figure/seg_pemp.png}}
\label{seg_pemp}

\caption{Visual comparison of segmentation results.}
\label{fig_seg_result}
\end{figure}


\subsection{Characteristics Analysis}
In this section, we analyze the characteristics of each sub-model of UEM in combination with the experimental results and visualization.

\begin{figure*}[!t]
\centering
\subfloat[Mask]{\includegraphics[width=2.2in]{Figure/aem_crop1.pdf}}
\label{Mask} 
\subfloat[Filter Response Curve]{\includegraphics[width=4.5in]{Figure/response.pdf}}
\label{response_fixed}


\caption{Visual comparison of masks of AEMs and response curves of WEMs. The mask is zoomed in for better visualization.}
\label{fig_UEMA_MASK}
\end{figure*}

\noindent {\bf{Amplitude Encoding Model.}} 
We extract the mask of AEM-P and one channel mask of AEM-I, as shown in Figure~\ref{fig_UEMA_MASK} (a). The AEM-I mask has a smaller range of values compared to the binary mask of AEM-P. Furthermore, the AEM-I mask exhibits a clear distinction from channel to channel, with neighboring channels having similar masks. For the full visualization of AEM-I masks, please refer to the supplement.


For AEM, it seems beneficial for achieving better spectral reconstruction with improved robustness to retain more scene information in optical encoding. Our experimental results suggest that optimizing masks of AEMs using a floating point instead of binary representation helps to improve spectral imaging performance.


%reconsruct network
\noindent {\bf{Phase Encoding Model.}} 
In PEM-I, it is difficult to get convergent optimization results if the PSF has the same size as the image. Therefore, we set the PSF size to 9, i.e., we only optimize the central 9*9 region and pad the rest area with 0. 
We visualize the PSFs of PEM-I that used two different decoding models in Figure~\ref{fig_freepsf}. The PSFs of the PEM-I with Res-U-Net are the most divergent and have the worst imaging performance. In contrast, the PSFs of the PEM-I with the Sim-Conv-Net experiment, which achieve the best performance, show a relatively concentrated pattern at the center with slight differences across channels. 

We conduct experiments with varying PSF sizes and convolutional kernel sizes of the decoding model, as shown in Table~\ref{table_p_psfkernel}. Figure~\ref{fig_FreePSF_size} visualizes these PSFs in RGB. The results indicated that smaller learnable PSF and kernel sizes in the decoding model can lead to greater convergence of PSF and improve performance. 

% Additional details can be found in the supplement.


In summary, for the PEM, it is necessary to design a concentrated PSF for a clear imaging quality while keeping a slight variance of the PSF across the channels to preserve some spectral information.

\begin{table}[!t]
  \centering
  \caption{Comparison of the imaging quality of systems using the PEM-I and the Sim-Conv-Net with different PSF and kernel size. The best result is marked in bold and the second-best result is underlined in each column.}
  \label{table_p_psfkernel}
  \resizebox{\linewidth}{!}{
  \begin{tabular}{ccccc}
  \hline
    \textbf{PSF Size} & \textbf{Kernel Size} & \textbf{PSNR$\uparrow$} & \textbf{PSNR-SI$\uparrow$} & \textbf{SAM$\downarrow$} \\ \hline
    3 & 3 & \textbf{44.75} & \textbf{38.69} & \textbf{0.0409} \\ 
    3 & 5 & 44 & 37.54 & 0.0421 \\ 
    3 & 7 & 42.43 & 35.57 & 0.0471 \\ 
    3 & 9 & 41.54 & 34.35 & 0.0483 \\ 
    9 & 3 & \underline{44.55} & \underline{38.32} & \underline{0.0417} \\ 
    9 & 5 & 44.01 & 37.47 & 0.0421 \\ 
    9 & 9 & 40.28 & 32.91 & 0.0512 \\ 
    9 & 15 & 34.14 & 26.52 & 0.0776 \\ 
    16 & 3 & 44.4 & 38.05 & 0.0419 \\ 
    16 & 5 & 40.43 & 33.33 & 0.0568 \\ 
    64 & 3 & 40.6 & 33.24 & 0.0509 \\ \hline
  \end{tabular}}
\end{table}



\begin{figure}[!t]
\centering
\captionsetup[subfloat]{labelsep=none,format=plain,labelformat=empty}
\subfloat[\scriptsize{Kernel Size: 3}]{\begin{overpic}[width=0.7in]{Figure/conv_patch_res_sim_3k_3p-psf-no-crop-rgb.png}
\put(-20,10){\scriptsize\rotatebox{90}{\color{black} PSF Size: 3}}
\end{overpic}}
\label{conv_patch_res_sim_3k_3p}
\subfloat[\scriptsize{Kernel Size: 5}]{\includegraphics[width=0.7in]{Figure/conv_patch_res_sim_5k_3p-psf-no-crop-rgb.png}}
\label{conv_patch_res_sim_5k_3p}
\subfloat[\scriptsize{Kernel Size: 7}]{\includegraphics[width=0.7in]{Figure/conv_patch_res_sim_7k_3p-psf-no-crop-rgb.png}}
\label{conv_patch_res_sim_7k_3p}
\subfloat[\scriptsize{Kernel Size: 9}]{\includegraphics[width=0.7in]{Figure/conv_patch_res_sim_9k_3p-psf-no-crop-rgb.png}}
\label{conv_patch_res_sim_9k_3p}

\subfloat[\scriptsize{Kernel Size: 3}]{\begin{overpic}[width=0.7in]{Figure/conv_patch_res_sim_3k_9p-psf-no-crop-rgb.png}
\put(-20,10){\scriptsize\rotatebox{90}{\color{black} PSF Size : 9}}
\end{overpic}}
\label{conv_patch_res_sim_3k_9p}
\subfloat[\scriptsize{Kernel Size: 5}]{\includegraphics[width=0.7in]{Figure/conv_patch_res_sim_5k_9p-psf-no-crop-rgb.png}}
\label{conv_patch_res_sim_5k_9p}
\subfloat[\scriptsize{Kernel Size: 9}]{\includegraphics[width=0.7in]{Figure/conv_patch_res_sim_9k_9p-psf-no-crop-rgb.png}}
\label{conv_patch_res_sim_9k_9p}
\subfloat[\scriptsize{Kernel Size:15}]{\includegraphics[width=0.7in]{Figure/conv_patch_res_sim_15k_9p-psf-no-crop-rgb.png}}
\label{conv_patch_res_sim_15k_9p}


\caption{Visual comparison of RGB PSFs of PEM-I with different sizes of learnable PSF and different convolutional kernel sizes of the decoding model.}
\label{fig_FreePSF_size}
\end{figure}

\noindent {\bf{Wavelength Encoding Model.}} 
In WEM-I, a linear layer is employed for encoding instead of a fixed RGB filter response function. We visualize the weights of the linear layer as spectral response curves for comparison with the FLIR BFS-U3-04S2C-C. As shown in Figure~\ref{fig_UEMA_MASK} (b), the response curve of the WEM-I is densely serrated, while the WEM-I with positive constraints  (WEM-I w/ P.C.) is smoother but still has more peaks than the ordinary camera's response curve. Comparing the performance of the three WEMs in Table~\ref{table_codedsensor}, the WEM-I still has the best imaging performance, while the WEM-I w/ P.C. and the WEM-P exhibit comparable imaging performance.

 
\begin{table}[!t]
  \centering
  \caption{Comparison of the imaging quality of systems using different types of WEM, where the WEM w/ P.C. represents the wavelength encoding model with positive constraints. The best result is marked in bold and the second-best result is underlined in each column.}
  \label{table_codedsensor}
  \resizebox{\linewidth}{!}
  {\begin{tabular}{ccccc}
  \hline
    \textbf{Encoding Model} & \textbf{PSNR$\uparrow$} & \textbf{PSNR-SI$\uparrow$} & \textbf{SAM$\downarrow$} & \textbf{ERGAS$\downarrow$} \\ \hline
    \textbf{WEM-I} & \textbf{45.25} & 38.51 & \textbf{0.0328} & \textbf{5.23} \\ 
    \textbf{WEM-P} & \underline{44.96} & \underline{38.81} & \underline{0.0399} & 6.23 \\ 
    \textbf{WEM-I w/ P.C.} & 44.26 & \textbf{38.84} & 0.0432 & \underline{5.37} \\ \hline
    
  \end{tabular}}
\end{table}

For the WEM, the response of the filter and the sensor plays a crucial role in the system since it controls the information bottleneck between the encoder and the decoder. When the response is optimized according to the task, the response curve will usually have multiple peaks. According to our results, the ideal shape of the filter response curve tends to have multiple separated sharp peaks compared to the ordinary response curves of cameras. Therefore, we suggest separating the peaks of the different response curves from each other as much as possible in designing to achieve better spectral imaging performance.


==> sec/5_conclusion.tex <==
\section{Conclusion}

In this study, we proposed the UEM which allows for a fair comparison of amplitude, phase, and wavelength encoding computational spectral imaging systems through joint encoder-decoder optimization. We utilized the UEM to establish physical models of these systems, enabling a comprehensive analysis of their performance. Additionally, we extend the UEM to ideal models and explore their potential upper bounds of performance without physical constraints. 
We also evaluated these systems on the spectral image segmentation task to investigate the correlation between low-level and high-level task performance. 
Finally, by visualizing and analyzing the ideal UEMs, we provided comprehensive suggestions and insights for the future design of spectral imaging systems.
